Efficient Signed Graph Sampling via Balancing & Gershgorin Disc Perfect Alignment

A basic premise in graph signal processing (GSP) is that a graph encoding pairwise (anti-)correlations of the targeted signal as edge weights is exploited for graph filtering. However, existing fast graph sampling schemes are designed and tested only for positive graphs describing positive correlations. In this paper, we show that for datasets with strong inherent anti-correlations, a suitable graph contains both positive and negative edge weights. In response, we propose a linear-time signed graph sampling method centered on the concept of balanced signed graphs. Specifically, given an empirical covariance data matrix $\bar{\bf{C}}$, we first learn a sparse inverse matrix (graph Laplacian) $\mathcal{L}$ corresponding to a signed graph $\mathcal{G}$. We define the eigenvectors of Laplacian $\mathcal{L}_B$ for a balanced signed graph $\mathcal{G}_B$ -- approximating $\mathcal{G}$ via edge weight augmentation -- as graph frequency components. Next, we choose samples to minimize the low-pass filter reconstruction error in two steps. We first align all Gershgorin disc left-ends of Laplacian $\mathcal{L}_B$ at smallest eigenvalue $\lambda_{\min}(\mathcal{L}_B)$ via similarity transform $\mathcal{L}_p = \S \mathcal{L}_B \S^{-1}$, leveraging a recent linear algebra theorem called Gershgorin disc perfect alignment (GDPA). We then perform sampling on $\mathcal{L}_p$ using a previous fast Gershgorin disc alignment sampling (GDAS) scheme. Experimental results show that our signed graph sampling method outperformed existing fast sampling schemes noticeably on various datasets.

==> learn.tex <==
%\red{Saghar: Please write about GLASSO (learning of a sparse inverse covariance matrix i.e., a signed graph) and positive graph learning fron Antonio's scheme, for example. }
We use two frameworks where graph learning is formulated as the estimation of different types of graph Laplacian matrices from data. 

To estimate a \textit{signed} (generalized) graph Laplacian matrix, given an empirical covariance matrix $\bar{\C}$ computed from data, we use the following GLASSO formulation \cite{articleglasso,mazumder2012graphical}:
\begin{align}
\min_\cL ~~ \text{Tr}(\cL \bar{\C}) -\log \det \cL + \rho \; \| \cL \|_1
\label{eq:glasso}
\end{align}
where $\rho > 0$ is a shrinkage parameter for the $l_1$-norm term.
We solve \eqref{eq:glasso} using a variant of the \textit{block Coordinate descent} (BCD) algorithm in \cite{wright2015coordinate}. 
% Specifically, we first solve the \textit{dual} of GLASSO as follows.
% We first note that the $l_1$ norm in \eqref{eq:glasso} can be written as 
% \begin{align}
%   \|\L\|_1 = \max_{\| \U \|_\infty\leq 1} ~~\text{Tr}(\L\U) 
% \end{align}
% where $\| \U \|_\infty$ is the maximum absolute value element of the symmetric matrix $\U$. 
% Then the dual problem of GLASSO that solves for an estimated covariance matrix $\C = \L^{-1}$ is
% %Denote by $\C = \P^{-1}$. 
% \begin{align}
% \min_{\C^{-1} \in \cH^+} ~~ -\log \det \C, 
% ~~~\mbox{s.t.} ~~ 
% \| \C - \bar{\C} \|_\infty \leq \rho
% \label{eq:glasso_dual}    
% \end{align}
% where $\C =\bar{\C}+\U$  implies that the primal and dual variables are related via $\L = {(\bar{\C}+\U)}^{-1} $ \cite{Banerjee7}. 
Specifically, we solve its dual iteratively by updating one row / column of dual variable $\C = \cL^{-1}$ till convergence. Here, by construction, $\cL$ is a \textit{positive definite} (PD) matrix.

% To solve \eqref{eq:glasso_dual}, 
% we update one row-column pair in $\C$ in \eqref{eq:glasso_dual} in each iteration. 
% Specifically, we first reorder the rows / columns of $\C$ so that the optimizing row / column are swapped to the last.
% We then partition $\bar{\C}$ and $\C$ into blocks: 
% \begin{align}
% \C = 
% \begin{pmatrix}
%     \C_{11} & \c_{12}\\
%     \c_{12}^\top & c_{22}
% \end{pmatrix},~~ 
% \bar{\C} =
% \begin{pmatrix}
%     \bar{\C}_{11} & \bar{\c}_{12}\\
%     \bar{\c}_{12}^\top & \bar{c}_{22}
% \end{pmatrix}
% \end{align}\noindent
% \cite{Banerjee7} showed that the optimal $\c_{12}$ is the solution to the following linearly constrained quadratic programming problem:
% \begin{align}
% \c_{12} = \text{arg}\,\min\limits_{\y}\, \{\y^\top\C_{11}^{-1}\y\},  ~~\mbox{s.t.} ~~ \| \y - \bar{\c}_{12} \|_\infty \leq \rho
% \label{eq:c12}
% \end{align}

% Our algorithm to solve \eqref{eq:glasso} is thus as follows.
% We minimize the GLASSO terms in \eqref{eq:glasso} by solving its dual \eqref{eq:glasso_dual}---iteratively updating one row / column of $\C$ using \eqref{eq:c12}.
% We then project $\L = \C^{-1}$ to convex cone $\cH_{\u}^+$ using our projection operator. 
% We repeat these two steps till convergence.
% Note that \textit{both steps are computed using covariance $\C$ directly}, and thus inversion to graph Laplacian $\L = \C^{-1}$ is not necessary until convergence, when we output a solution.


To estimate a combinatorial graph Laplacian matrix corresponding to a \textit{positive} graph, we use the formulation in \cite{egilmez17}. 
%\red{but a combinatorial graph Laplacian matrix is PSD and not invertible. something is not precise here.}
Specifically, we formulate the following optimization
\begin{equation}
\min_\L ~~  \text{Tr}(\L \K) -\log |\L| ~~ \text{subject to} ~~ \L \in \cL_c(\A)
\label{cgl}
\end{equation}
where $\K=\bar{\C}+\F$, $\F$ is the regularization matrix defined as $\F = \rho (2\I - \1 \1^{\top})$, $\A$ is the connectivity matrix, and the set of constraints $\cL_c(\A)$ restricts $\L$ to a combinatorial graph Laplacian matrix. 
%\blue{The $l_1$-norm term with parameter $\rho$ can be written as $\rho \; \| \L \|_1 = \text{Tr}(\L \F)$ where $\F = \rho\;(2\I - \1\1^\top)$.}
Since $\L$ is a \textit{positive semi-definite} (PSD) matrix with eigenvalue $0$, $|\L|$ is the pseudo-determinant.
Considering the graph connectivity is unknown, $\A$ is set to represent a fully connected graph, \ie, $\A = \A_\text{full} = \1\1^\top - \I$.
See \cite{egilmez17} for details on how \eqref{cgl} is computed.
